On the Counting Sequence of Z-convex Polyominoes

The degree of convexity of a convex polyomino P is the smallest integer k such that any two cells of P can be joined by a monotone path inside P with at most k changes of direction. In this paper, we present a set of formulas and equations that are the basis of a C++ program that allows you to compute the longest counting sequence known to date (with respect to the area) of convex polyominoes of degree of convexity at most 2

==> eptcsdata.tex <==
\providecommand{\firstpage}{57}
\providecommand{\publicationstatus}{S. Brlek and L. Ferrari (Eds.): GASCom 2026\\
EPTCS 445, 2026, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.445.8}{10.4204/EPTCS.445.8}}
\pdfoutput=1

